Infrastructure Quality Assessment in Africa using Satellite Imagery and Deep Learning

The UN Sustainable Development Goals allude to the importance of infrastructure quality in three of its seventeen goals. However, monitoring infrastructure quality in developing regions remains prohibitively expensive and impedes efforts to measure progress toward these goals. To this end, we investigate the use of widely available remote sensing data for the prediction of infrastructure quality in Africa. We train a convolutional neural network to predict ground truth labels from the Afrobarometer Round 6 survey using Landsat 8 and Sentinel 1 satellite imagery. Our best models predict infrastructure quality with AUROC scores of 0.881 on Electricity, 0.862 on Sewerage, 0.739 on Piped Water, and 0.786 on Roads using Landsat 8. These performances are significantly better than models that leverage OpenStreetMap or nighttime light intensity on the same tasks. We also demonstrate that our trained model can accurately make predictions in an unseen country after fine-tuning on a small sample of images. Furthermore, the model can be deployed in regions with limited samples to predict infrastructure outcomes with higher performance than nearest neighbor spatial interpolation.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g copyright statements.

==> cs325b_report_bs_oresp.tex <==
\subsection{Predicting From Other Responses (Oracle)}
\noindent To get a better sense of ideal model performance, we also constructed an `oracle' baseline. In this baseline, we use all other observed variables in the data to predict one held-out variable. For illustration, consider predicting an enumeration area's access to piped water from its access to sewerage, electricity, roads, etc. For consistency throughout the analysis, we ran this model using the binary variables (e.g. electricity, sewerage, and piped water) of Afrobarometer, predicting each binary variable using all other binary variables. Splitting the data into 80\% training validation, and 20\% testing, we find that some infrastructure categories have high predictability even from using simple logistic regression. Table\ref{cs325b:table:bs:other_resp:metric} displays the relevant metrics for some categories. 
\\\\
\noindent The results here perform very well, but they represent an ideal, as they still depend on survey data from each enumeration area. We believe that the high scores are due to high correlation between the different survey response variables. Additionally, we tried SVM and random forest on the same dataset, with resulting performance more or less similar to that of logistic regression.    

==> cs325b_report_bs_osm.tex <==
\subsubsection{OSM}
\noindent As OSM is highly related to infrastructure, we decided to use a simple OSM baseline model for comparison purposes.  Using the previously mentioned metrics of \emph{accuracy}, \emph{precision}, \emph{recall}, \emph{f1-score}, and (\emph{\textbf{AUROC}}), we ran logistic regression on a set of input features. The features were various transformations of the number of highways and number of buildings in OSM in a given enumeration area. Feature transformation and normalization ensures that input data is similarly scaled. The transformations from raw inputs to the post-processed inputs (denoted as $\phi(x)$) are illustrated in following Table~\ref{cs325b:table:osm:bs:feat_trans} with accompanying interpretations. 
\begin{table}[hpbt]
\centering
\caption{Feature transformation}
\label{cs325b:table:osm:bs:feat_trans}
\begin{tabular}{ccc}
\hline
feature & transformation & interpretation \\
\hline
\hline 
$\phi_1(x)$ & $x_1$ & hwy \# \\
$\phi_2(x)$ & $x_2$ & bldg \# \\
$\phi_3(x)$ & $\log x_1$ & utility of hwy  \\
$\phi_4(x)$ & $\log x_2$ & utility of bldg  \\ 
$\phi_5(x)$ & $\frac{x_1}{x_2}$ & ratio of hwy per bldg \\
$\phi_6(x)$ & $\sqrt{x_1}$ & hwy \# along distance (km) \\
$\phi_7(x)$ & $\sqrt{x_2}$ & bldg \# along distance (km) \\
\hline 
\end{tabular}
\end{table}
% For logistic regression we simply fit the model 
% \begin{align}
% & \log(\frac{p}{1-p}) = \sum_{i=1}^K w_i\phi_i(x) + \gamma \sum_{i=1}^K |w_i | + \beta \sum_{i=1}^K w_i^2  \\ 
% & = \mathbf{w}^T\phi(x) + \gamma \|\mathbf{w}\|_1 + \beta\|\mathbf{w}\|_2^2
% \end{align}
% where $p = P(Y=1| \phi(x))$, $Y$ is our response label, $K$ is number of features, $\mathbf{w} \in R^{K}$ are weights, and $\gamma, \beta$ are tuning parameters.
\\
We display results in Table~\ref{cs325b:table:osm:metric:result}, truncated to only include variables whose AUROC is larger then 0.6. We also conducted experiments using Support Vector Machine (SVM) and a random forest, finding similar performance compared with logistic regression. %Figure ~\ref{cs325b:fig:roc:osm} depicts the \emph{auroc} metric for all binary response variables. 
\\\\
\noindent With AUROCs in the range of 0.7, results indicate meaningful yet limited predictive power. Precision and recall numbers greater than 0.5 indicate that the model is actively making predictions. For those categories that accuracies are not much higher than the balance of the predicted variable, it indicates that these predictions are moderately better than random guessing and close to the prior distribution of the response variables. We find this is reasonable given the nature of OSM as an infrastructure related dataset that is both incomplete and with features that are potentially less correlated with certain infrastructure measures.





==> cs325b_report_dat_osm.tex <==
\subsection{OpenStreetMap Data}
\noindent OpenStreetMap(OSM) is an open-source mapping project based on volunteer-supplied cartographic and infrastructure information from around the world. OSM is open source, and humanitarian teams have used it extensively in health outreach projects, particularly in Africa. Consequently, OSM has the most complete coverage of road conditions of any major mapping projects, including commercial map engines such as Google maps\cite{HumanOSMTeam,Zhao2016report}. OSM includes measures beyond the presence of roads, such as buildings and road-type. It should be noted that while OSM is extensive, it is not exhaustive in the same as satellite imagery and relies on human inputted values. 
\\\\
\noindent OSM encodes roads as 'ways' that connect a collection of 'nodes'. Each node has an associated latitude and longitude, and includes other associated metadata, such as number of proximate buildings. In our usage of OSM, we align survey data with an appropriately sized area in OSM. Similarly as with satellite data, not every survey point had associated OSM data, but there were sufficient records to run our baseline model.

%OSM encodes streets as ways representing a collection of nodes. Each node has an ID, longitude/latitude coordinates, and tags, or the metadata associated with each node/ways. One advantage of OSM is the availability of metadata associated with different kinds of infrastructures, e.g. highways, buildings, etc. In order to align with the geo-location provided in the survey response, we fetch the associated highway and building information by those targeted locations. And we zoom in the map area around $2km \times 2km$. There are 6833 valid records after we processed the raw data that is queried through OSM api, due to some data retrieval and lack of information error. But this ample resource can already provide a good baseline model for us to understand the predictability of the infrastructure related response variables.         
